Measuring Gender Bias in Word Embeddings of Gendered Languages Requires Disentangling Grammatical Gender Signals

Does the grammatical gender of a language interfere when measuring the semantic gender information captured by its word embeddings? A number of anomalous gender bias measurements in the embeddings of gendered languages suggest this possibility. We demonstrate that word embeddings learn the association between a noun and its grammatical gender in grammatically gendered languages, which can skew social gender bias measurements. Consequently, word embedding post-processing methods are introduced to quantify, disentangle, and evaluate grammatical gender signals. The evaluation is performed on five gendered languages from the Germanic, Romance, and Slavic branches of the Indo-European language family. Our method reduces the strength of grammatical gender signals, which is measured in terms of effect size (Cohen's d), by a significant average of d = 1.3 for French, German, and Italian, and d = 0.56 for Polish and Spanish. Once grammatical gender is disentangled, the association between over 90% of 10,000 inanimate nouns and their assigned grammatical gender weakens, and cross-lingual bias results from the Word Embedding Association Test (WEAT) become more congruent with country-level implicit bias measurements. The results further suggest that disentangling grammatical gender signals from word embeddings may lead to improvement in semantic machine learning tasks.

==> pics/flowchart.tex <==
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\begin{tikzpicture}[node distance=2cm]
\node (start) [startstop] {Start};
\node (in1) [io, below of=start] {Input};
\node (pro1) [process, below of=in1] {Process 1};
\node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};
\node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
\end{tikzpicture}


==> tables/baseline-gg-weat-d1.tex <==
\begin{table}[h!]
\begin{center}
\centering
\begin{tabular}{c|p{6mm}|p{7mm}ccp{5mm}p{4mm}c}
\hline
\textbf{Test}& \textbf{Lang} & \textbf{WEAT} & \pmb{$d_{init}$} & \pmb{$d_{1}$} & \pmb{$d_{SVC}$} & \pmb{$p_{SVC}$} & \pmb{$\Delta$} \\
\midrule
Baseline & EN & FloI & 1.45 & -- & -- & -- & -- \\ \cline{3-8}
& &InsW & 1.54 & -- & -- & -- & -- \\ 
\cline{2-8}
& FR & FloI & 1.38 & 1.35 & 1.44 & $10^{-3}$ & +0.06 \\ \cline{3-8}
&& InsW & 1.40 & 1.43 & 1.45 & $10^{-6}$ & +0.05 \\ 
\cline{2-8}
&DE &  FloI & 1.58 & 1.60 & 1.62 & $10^{-5}$ & +0.04 \\ \cline{3-8}
& & InsW & 1.63 & 1.64 & 1.67 & $10^{-9}$ & +0.04 \\ 
\cline{2-8}

& IT & FloI & 1.56 & 1.56 & 1.61 & $10^{-4}$ & +0.05 \\ \cline{3-8}
& & InsW & 1.42 & 1.44 & 1.37 & $10^{-6}$ & -0.05\\ 
\cline{2-8}

& PL & FloI &  1.00 & 1.07 & 1.34 & $10^{-3}$ & +0.34\\ \cline{3-8}
& & InsW &  0.71 & 0.80 & 1.19 & $10^{-5}$ & +0.48 \\ 
\cline{2-8}

& ES & FloI & 1.67 & 1.59 & 1.60 & $10^{-4}$ & -0.07 \\ \cline{3-8}
& & InsW & 1.08 & 0.99 & 1.12 & $10^{-4}$ & +0.04 \\ 
\hline 
Grammatical & FR & GG & 1.82 & 1.38 & 0.40 & 0.20 &  -1.42 \\ 
\cline{2-8}

Gender &DE &  GG & 1.55 & 1.04 & 0.30 & 0.26 & -1.25 \\ 
\cline{2-8}

Evaluation & IT & GG & 1.79 & 1.52 & 0.58 & 0.11 & -1.21\\ 
\cline{2-8}

& PL & GG &  1.85 & 1.77 & 1.34 & $10^{-3}$ & -0.51\\ 
\cline{2-8}

& ES & GG & 1.83 & 1.55 & 1.23 & $10^{-3}$ & -0.60 \\ 
\hline 
\end{tabular}
\caption{\label{tab:main-results}
{Baseline and evaluation WEAT results before and after disentangling grammatical gender with SVC. $d_{init}$ denotes the initial effect size (magnitude of bias measured in Cohen's $d$), $d_{1}$ is effect size after 1 iteration, and $d_{SVC}$ refer to effect size after disentangling grammatical gender. $p$ is a measure of statistical significance, $\Delta$ measures the change in effect size ($d_{SVC}-d_{init}$).}} 
\end{center}
\end{table}

==> tables/gender-weat-d1.tex <==
\begin{table}
    \centering
    \begin{tabular}{p{5mm}ccccp{4mm}cp{4mm}c}
         \hline
         \textbf{Lang} & \textbf{WEAT} & \pmb{$d_{init}$} & \pmb{$d_{1}$} & \pmb{$d_{SVC}$} & \pmb{$p_{SVC}$} & \pmb{$\Delta$} & \pmb{$d_{IAT}$} & \pmb{$C\textsuperscript{*}$}\\
        \midrule
        EN &  GenS & 0.88 & -- & -- & -- &  -- & 0.38 & -- \\   
        & GenC & 1.66 & -- & -- & -- & -- & 0.38 & -- \\
        \hline
        FR & GenS & 0.30  & 0.43 & 0.43 & 0.10 & +0.13 & 0.42 & \checkmark\\
        & GenC & 0.77 & 1.12 & 1.14 & 0.01 & +0.37 & 0.38 & \checkmark \\
        \hline
        DE &  GenS & 0.50 & 0.74 & 0.69 & 0.02 & +0.19 &0.42 & \checkmark\\
        & GenC  & 0.85 & 0.93 & 0.91 & 0.03 &  +0.06 & 0.40 & \checkmark\\
        \hline
        IT & GenS & -0.01 & 0.05 & 0.35 & 0.15 & +0.36 & 0.39 & \checkmark \\
        & GenC & 0.75 & 1.06 & 0.91 & 0.03 & +0.16 & 0.41 & \checkmark \\
        \hline
        PL & GenS & -0.26 & -0.17 & -0.07 & 0.58 & +0.19 & 0.49 & -- \\
        & GenC & 0.59 &  0.80 & 0.91 & 0.03 & +0.32 & 0.36 & \checkmark \\
        \hline
        ES & GenS & -0.32 & -0.12 & 0.04 & 0.46 & +0.36 & 0.33 & -- \\ 
        & GenC & 1.31 & 1.49 & 1.52  & $10^{-3}$ &  +0.21 & 0.35 & \checkmark \\
        \hline 
    \end{tabular}
    \caption{Gender WEAT results before and after disentangling grammatical gender with SVC. $d_{init}$ denotes the initial effect size (magnitude of bias measured in Cohen's $d$), $d_{1}$ is effect size after 1 iteration and $d_{SVC}$ refers to effect size after disentangling grammatical gender. $p$ is a measure of statistical significance, $\Delta$ measures the change in effect size ($d_{SVC}-d_{init}$). $d_{IAT}$ denotes the ground truth effect sizes reported by \citep{PMID:32747806} for GenC and \citep{Nosek10593} for GenS. \pmb{$ C\textsuperscript{*}$} stands for congruent, which denotes whether $d_{SVC}$ matches in sign with $d_{IAT}$.}
    \label{tab:gender_weat}
\end{table}
